The NANOGrav Nine-year Data Set: Limits on the Isotropic Stochastic Gravitational Wave Background

We compute upper limits on the nanohertz-frequency isotropic stochastic gravitational wave background (GWB) using the 9-year data release from the North American Nanohertz Observatory for Gravitational Waves (NANOGrav) collaboration. We set upper limits for a GWB from supermassive black hole binaries under power law, broken power law, and free spectral coefficient GW spectrum models. We place a 95\% upper limit on the strain amplitude (at a frequency of yr$^{-1}$) in the power law model of $A_{\rm gw} < 1.5\times 10^{-15}$. For a broken power law model, we place priors on the strain amplitude derived from simulations of Sesana (2013) and McWilliams et al. (2014). We find that the data favor a broken power law to a pure power law with odds ratios of 22 and 2.2 to one for the McWilliams and Sesana prior models, respectively. The McWilliams model is essentially ruled out by the data, and the Sesana model is in tension with the data under the assumption of a pure power law. Using the broken power-law analysis we construct posterior distributions on environmental factors that drive the binary to the GW-driven regime including the stellar mass density for stellar-scattering, mass accretion rate for circumbinary disk interaction, and orbital eccentricity for eccentric binaries, marking the first time that the shape of the GWB spectrum has been used to make astrophysical inferences. We then place the most stringent limits so far on the energy density of relic GWs, $\Omega_\mathrm{gw}(f)\,h^2 < 4.2 \times 10^{-10}$, yielding a limit on the Hubble parameter during inflation of $H_*=1.6\times10^{-2}~m_{Pl}$, where $m_{Pl}$ is the Planck mass. Our limit on the cosmic string GWB, $\Omega_\mathrm{gw}(f)\, h^2 < 2.2 \times 10^{-10}$, translates to a conservative limit of $G\mu<3.3\times 10^{-8}$ - a factor of 4 better than the joint Planck and high-$l$ CMB data from other experiments.

==> dis.tex <==

\subsection{Astrophysical Model Limits}
While the parameter estimation of the previous section is interesting in and of itself, some of the most interesting science available from the NANOGrav data is accessible only by relating these parameters to properties of the source populations.
In Section \ref{sec:joesarah} we use the results of our power-law analyses of Section \ref{sec:power-spectral-limits} to provide constraints on the parameters of scaling relations between host galaxies and black holes. We then go beyond the assumption of a power-law spectrum in Section \ref{sec:environs} to investigate how our constraints on the shape of the characteristic strain spectrum from Section \ref{sec:AstrophysicalModel} map to constraints on the environment of SMBH binaries. Finally in Section \ref{sec:eccentricity}, we probe the eccentricity of binaries before they entered the PTA band. 

\subsubsection{Constraints on Host Galaxy -- Black Hole Scaling Relations}
\label{sec:joesarah}
If the gravitational wave spectrum is assumed to be created by an ensemble of binary SMBHs that are formed following galaxy mergers (spectral index of $-2/3$), and whose evolution is assumed to be dominated by GW emission throughout the PTA-sensitive waveband, then we can trace the expected binary SMBH population using known observations of galaxy merger rates, the galaxy stellar mass function, and the black hole-host galaxy relation. This is the approach taken in the models of \citetalias{s13}, \cite{rws+15}, and \cite{ss15}. Assuming equal fractional uncertainties in these parameters, the black hole-host galaxy relation will have the largest impact on the predicted level of the GWB background. This is due to a much stronger dependence on the chirp mass of each source than on the number of sources, $h_c equation?$.

\cite{mdf+15} show that it is difficult to extract information from PTA limits without making significant assumptions about the shape of the binary black hole merger rate density. If instead a galaxy merger rate density calculated from observed galaxy parameters is used as a proxy, then a limit on the GWB background can be directly translated into a limit on the input galaxy parameter spaces \citep{ss15}. Since observations of the galaxy merger rate rely heavily on theoretical modeling of the galaxy merger timescale, the scaling between host galaxy properties and black hole mass (e.\,g.\,~\cite{hr04}, \cite{mm13}) is the `observed' parameter that is most easily constrained by NANOGrav data. Specifically, we constrain the $M_{\bullet}-M_{\rm bulge}$ relation:
%\cite{ss15} argue that when using observed galaxy parameters as a proxy for the binary black hole merger rate density, the black hole-host galaxy relation is the `observed' quantity with the largest impact on these model's predictions on the strength of the GWB background. This is also shown in \cite{something sesana} and is largely due to the relative scaling of the GWB background with respect to mass and number of sources. \cite{rws+15} shows that the galaxy merger rate is at least equally unconstrained observationally in these models, however observational constraints on the galaxy merger rate rely heavily on theoretical modeling of the galaxy merger timescale, which is not well known at this time.  However, recent simulations by \cite{Lotz et al?} provide something closer to reality, which makes current observational measurements of the galaxy merger rate more constrained than in the past \citep{conselice14 - check this}. 
%Observations of the galaxy merger rate and the galaxy stellar mass function are largely constrained, and their uncertainties have only minor impact on the strength of the GWB \citep{ss15}. In contrast, the scaling between host galaxy properties and black hole mass (e.\,g.~\cite{hr04}, \cite{mm13}) has a much larger impact, and can be constrained by NANOGrav data. Specifically, we constrain the $M_{\bullet}-M_{\rm bulge}$ relation:
%For this analysis we use the approach laid out by \cite{ss15}. The model of \cite{ss15} is similar to the models in \citetalias{s13} and \citetalias{rws+14}, described in Sec. \ref{sec:power-spectral-limits}. In brief, we use two leading measurements of the galaxy stellar mass function, \cite{isl+10} and \cite{tqt+14}, and two measurements of the galaxy merger rate, \cite{rdd+14} and \cite{kfp+14}, as the basis for simulating a local population of binary SMBHs. Those two functions are largely constrained by observation, and their uncertainties have only minor impact on the strength of the GWB. A much larger impact, however, is the scaling between host galaxy properties and black hole mass (e.\,g.~\cite{hr04}, \cite{mm13}):
\be
\label{eq:M-M_bulge}
{\rm log}_{10} M_{\bullet} = \alpha + \beta ~{\rm log}_{10} \left( M_{bulge} / 10^{11} M_{\odot} \right)~.
\ee
In addition to $\alpha$ and $\beta$, observational measurements of this relation also fit for $\epsilon$, the intrinsic scatter of individual galaxy measurements around the common $\alpha$, $\beta$ trend line.  In practice, $\alpha$ and $\epsilon$ have the greatest impact on predictions of $A_{\rm gw}$, and all observational measurements agree that $\beta \approx 1$.

PTAs are most sensitive to binary SMBHs where both black holes are $\gtrsim$10$^8\msun$ (e.g. \cite{svc08}). Therefore $M_{\bullet}-M_{bulge}$ relations that are derived including the most massive systems are the most relevant to understanding the population in the PTA band. Several recent measurements of the $M_{\bullet}-M_{bulge}$ relation specifically include high-galaxy-mass measurements, e.g. those from Brightest Cluster Galaxies (BCGs). As these fits include the high-mass black holes that we expect to dominate the PTA signals, we take these as the ``gold standard" for comparison with PTA limits \citep[e.g.]{kh13, mm13}.

The translation of an upper limit on $A_{\rm gw}$ to the black hole-host galaxy parameter space is calculated as follows: 
\be
p \left( \alpha, \beta, \epsilon | {\rm PTA} \right) \propto \int d\theta ~p(\theta) ~p(A_{\rm gw} ( \alpha, \beta, \epsilon, \theta ) | {\rm PTA}) ,
\ee
where the posterior of $A_{\rm gw}$, $p \left( A_{\rm gw} (\alpha, \beta, \epsilon, \theta) | {\rm PTA} \right)$, is the marginalized posterior distribution of $A_{\rm gw}$, which is shown in Fig. \ref{fig:9-5-amplitude}; $A_{\rm gw} \left( \alpha, \beta, \epsilon, \theta \right)$ is the prediction of $A_{\rm gw}$ calculated from the model in \cite{ss15}; $\theta$ represents the galaxy stellar mass function and the galaxy merger rate; and $p \left( \alpha, \beta, \epsilon | {\rm PTA} \right)$ is the marginalized posterior distribution of the black hole-host galaxy relation, which is shown in Fig. \ref{fig:a-b-e-triplot}. For this analysis, we use two leading measurements of the galaxy stellar mass function, \cite{iml+13} and \cite{tqt+14}, and two measurements of the galaxy merger rate, \cite{rdd+14} and \cite{kfp+14}, as the basis for simulating a local population of binary SMBHs. As seen in Fig. \ref{fig:a-b-e-triplot}, $\beta$ is not informed by a PTA posterior, but the combination of $\alpha$ and $\epsilon$ are, with the strongest limit being set on $\alpha$.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/a-b-e-triplot.pdf} 
\caption{The above plot shows the translation of the marginalized posterior distribution of $A_{\rm gw}$ into the black hole-host galaxy parameter space, which is characterized by an intercept $\alpha$, a slope $\beta$, and an intrinsic scatter $\epsilon$. $\beta$ is not informed by the distribution of $A_{\rm gw}$, while both $\alpha$ and $\epsilon$ are, with a limit on $\alpha$ being more strongly set. The curves show the 1, 2, and 3$\sigma$ contours. Relevant observational measurements are also shown, with \cite{mm13} in blue and \cite{kh13} in magenta. Since $\beta$ is not strongly informed by the upper limit, we can set an upper limit in $\alpha$-$\epsilon$ space by marginalizing over $\beta$. This upper limit is shown in Fig. \ref{fig:alpha-epsilon}.}
\label{fig:a-b-e-triplot}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/alphavsepsilon.pdf} 
\caption{The above plot shows the translation of the $95\%$ upper limit on $A_{\rm gw}$ into the parameter space $\alpha$-$\epsilon$, which characterizes the black hole-host galaxy relation as described in Equation. \eqref{eq:M-M_bulge}. The points above the line are inconsistent with the model described in \cite{ss15}. Observed values of these parameters are shown with errorbars.}
\label{fig:alpha-epsilon}
\end{figure}

Fig. \ref{fig:alpha-epsilon} shows the translation of the NANOGrav upper limit into $\alpha$-$\epsilon$ parameter space with observational measurements of the parameters from \cite{kh13} and \cite{mm13}. There is a slight inconsistency between the NANOGrav upper limit and the \cite{kh13} measurement, while the \cite{mm13} measurement appears to be consistent with the current upper limit.  Potential solutions to an inconsistency include: a significant number of black hole binaries do not reach the GW-dominant regime in our assumed timescale (they ``stall"); the `classical' assumption of a power-law strain spectrum in the PTA band is incorrect and in fact there is a turn-over in the strain spectrum at lower frequencies (see Sec. \ref{sec:AstrophysicalModel}); or that the measured astronomical parameters are not correct for the population of binary SMBHs in the PTA band.

As the possibility for a different strain spectrum curve is discussed elsewhere in this paper, let us explore the potential for `stalling' within the assumptions of the models in \citetalias{s13} and \cite{ss15}.
there is an implicit assumption that binary SMBHs begin radiating GWs in the PTA band at the same cosmological time as the galaxy merger. While observational measurements of the galaxy merger rate take into account a merger timescale, which is essentially a dynamical friction timescale, there is nothing in the model to allow for anything other than an efficient solution to the `last-parsec' problem \citep{bbr80}. As done in \cite{ss15}, we introduce a variable, $T_{\rm stall}$, which is a measure of the time between the galaxy merger and the binary SMBH entering the PTA band. Fig \ref{fig:Tstall} shows the translation of the posterior distribution of $A_{\rm gw}$ into a probability distribution of $T_{\rm stall}$ assuming the measured values for the host galaxy-black hole relation from \cite{kh13}. We set a $95\%$ lower limit on $T_{\rm stall}$ of 0.73 Gyr if the \citet{kh13} $M_{\bullet}-M_{bulge}$ relation is correct.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/Tstall_UpLim.pdf} 
\caption{In the above plot, we allow $T_{\rm stall}$ to vary while holding $\alpha$, $\beta$, and $\epsilon$ constant at the measured values from \cite{kh13}. The probability of $T_{\rm stall}$ is a direct translation of the $95\%$ upper limit on $A_{\rm gw}$. We set a lower limit on $T_{\rm stall}$ of 0.73 Gyr, which is a measure of the time between the galaxy merger and the SMBH binary entering the PTA band.}
\label{fig:Tstall}
\end{figure}

\subsubsection{Constraints on binary environmental influences}
\label{sec:environs}

The cores of galactic merger remnants can harbor stars with little angular momentum and almost radial trajectories which intersect the central galactic region (centrophilic orbits). These stars can undergo three-body interactions with the resident supermassive black-hole binary, causing the stars to be ejected, which results in energy and angular momentum being extracted from the black hole system, and leading to binary hardening \citep{q96}.\footnote{We ignore the subtleties of loss-cone (the region of phase space populated by stars with centrophilic orbits) replenishing, and assume that all galactic merger remnants maintain the same mass density of core stars throughout the binary merger.} Additionally, the formation of circumbinary gaseous disks can lead to interactions which extract energy and angular momentum from the binary orbit, driving it towards smaller orbital separations \citep{ipp99}. We expect that, in the type of gas-poor galaxies which dominate the nanohertz GW signal, hardening from stellar scattering will dominate over circumbinary interactions, but we consider both in the following. We begin with a discussion of how these environmental mechanisms drive the evolution of the binary, then provide constraints on the frequency at which the characteristic strain spectrum exhibits a turnover from the analysis in Sec.\ \ref{sec:AstrophysicalModel}. We finish by mapping these frequencies to constraints on the astrophysical environment of SMBH binaries emitting GWs in the nanohertz band. 

\paragraph{Environmentally-driven orbital evolution}

We use the formalism of \citet{q96} to define the evolution of a (circular) binary due to three-body stellar scattering events, where
\be 
\frac{{\rm d}}{{\rm d}t}\left(\frac{1}{a}\right) = \frac{G\rho H}{\sigma},
\ee
where $a$ is the binary orbital semi-major axis, $\rho$ is the mass density of galactic core stars, $H$ is a dimensionless hardening rate which takes a value of $\sim 15$, and $\sigma$ is the velocity dispersion of core stars. Using Kepler's third law, we can rearrange this equation to solve for the rate of orbital frequency evolution, which gives ${\rm d}f/{\rm d}t \propto f^{1/3}$. Since the binary orbital evolution will be due to a combination of environmental influences and GW emission, ${\rm d}f/{\rm d}t$ is actually a sum over all mechanisms, as in Eq.\ (\ref{eq:evolve-sum}). We know that the rate of frequency evolution due to GW emission is ${\rm d}f/{\rm d}t \propto f^{11/3}$ \citep{pm63}, hence, in the language of the parametrized spectrum model in this paper given in Eq.\ (\ref{eq:turnover}), $\kappa=10/3$ for binary hardening by three-body stellar scattering. 

Likewise, the evolution of a circular binary due to circumbinary disk interaction is modeled within the $\alpha$-disk formalism \citep{ipp99,hkm09,s13c} as
\be
\frac{{\rm d}a}{{\rm d}t} = -\frac{2\dot{M}_1}{\mu}(aa_0)^{1/2},
\ee
where $\dot{M}_1$ is the accretion rate onto the primary black hole, $\mu$ is the binary reduced mass, and $a_0$ is a characteristic orbital separation at which the enclosed disk mass equals the mass of the secondary black hole. The latter can be expressed as \citep{ipp99}
\begin{align}
a_0 =&\,\, 3\times 10^3 \left(\frac{\alpha}{10^{-2}}\right)^{4/7}\left(\frac{M_2}{10^6 M_\odot}\right)^{5/7}\ \nonumber\\
&\times\left(\frac{M_1}{10^8 M_\odot}\right)^{-11/7}\left(100\frac{\dot{M_1}}{\dot{M_\mathrm{E}}}\right)^{-3/7}r_g,
\end{align}
where $\alpha$ is a disk viscosity parameter, $M_{1,2}$ are the binary black hole masses, $\dot{M_\mathrm{E}}$ is the Eddington accretion rate of the primary, and $r_g$ is the Schwarzschild radius of the primary. 

As in the stellar scattering case, we can rearrange this equation to determine the orbital frequency evolution. In this model, ${\rm d}f/{\rm d}t\propto f^{4/3}$, and so $\kappa=7/3$ for $\alpha$-disk binary interactions.

\paragraph{Constraints on spectral turnover frequency}
We define the spectral turnover frequency in the obvious way to mean the frequency at which the characteristic strain spectrum exhibits a change in slope. If the low-frequency slope is positive, this will correspond to the point at which the spectrum is maximized. One must note that setting $f=f_{\rm bend}$ in Eq.\ (\ref{eq:turnover}) does not maximize the characteristic strain spectrum. Rather the turnover frequency will be a function of both $f_{\rm bend}$ and $\kappa$:
\be
\label{eq:max-freq}
f_{\rm turn} = f_{\rm bend}\left(\frac{3\kappa}{4}-1\right)^{1/\kappa}.
\ee
We can combine our measurements of $f_\mathrm{bend}$ and $\kappa$ from the analysis in Sec.\ \ref{sec:AstrophysicalModel} to compute the probability distribution of spectral turnover frequencies. We find that placing numerical constraints on $\fbend$ is difficult as the posterior is heavily influenced by the prior, namely the upper and lower bounds for the uniform priors used in this analysis. In the following analysis we set the lower bound on $\fbend$ by requiring that the power at $f=1/T_{\rm span}$ differs by no more than 10\% from a pure-power-law for any value of $\kappa$. By using this prior, we ensure that we can recover a pure-power law spectrum (in our frequency range) for any value of $\kappa$. The upper bound of $\fbend$ is chosen based on the specific environmental coupling mechanism we are considering.

We emphasize that the probability
distributions of $f_\mathrm{bend}$, $\kappa$, and $f_\mathrm{turn}$ are not distributions of these parameters over the SMBH binary population. Rather our posterior distribution is illustrating the spread of our beliefs in the measurement of the single $f_\mathrm{bend}$ and $\kappa$ model parameters. 

% 
%\begin{table}
%\begin{center}
%\caption{\label{tab:fbend-fmax} Spectral bend and turnover frequency constraints. Limits correspond to the $95\%$ lower limit deduced from posterior probability distributions. Turnover frequencies are computed using the subset of posterior samples which have $\kappa>4/3$.}
%\input{fbend_fmax_table}
%\end{center}
%\end{table}
%

\paragraph{Constraints on environmental parameters}
We can now extract astrophysical constraints from our constraints on the transition and spectral turnover frequencies. By equating the rate of orbital evolution, ${\rm d}a/{\rm d}t$, due to environmental mechanisms and GW emission, we can deduce the characteristic transition frequency, $f_{\rm bend}$, between these influences. We firstly consider stellar-scattering, for which the transition frequency is given by

\begin{align}
\label{eq:fbend_stars}
f_\mathrm{bend} &= 3.13~\mathrm{nHz}\times\sigma^{-3/10}_{200} \rho^{3/10}_3 H^{3/10}_{15} M^{-2/5}_8 q^{-3/10}_r \\
&= 3.25~\mathrm{nHz}\times \rho_3^{3/10} H_{15}^{3/10}
M_8^{-23/50} q_r^{-3/10}
\end{align}
where $M$ is the total binary mass, $M_8 \equiv M / (10^8~\Msun)$, $q=M_2/M_1$, $q_r=q/(1+q)^2$, $\sigma_{200} \equiv
\sigma/(200~\mathrm{km/s})$, $\rho_3 \equiv \rho /
(10^3~\Msun\mathrm{pc}^{-3})$, and $H_{15} \equiv H / 15$. In the second line we have used the $M-\sigma$ relation.




==> fbend_fmax_table.tex <==
\begin{tabular}{lcccc}
\hline\hline
& \multicolumn{2}{c}{\citet{mop14} prior} & \multicolumn{2}{c}{\citet{s13} prior} \\
 & $f_\mathrm{bend}$ [nHz] & $f_\mathrm{turn}$ [nHz] &  $f_\mathrm{bend}$ [nHz] & $f_\mathrm{turn}$ [nHz] \\
\hline
Marginalized $\kappa$ & $13.6$  & $12.6$ & $5.29$ & $4.98$ \\
$\kappa=10/3$ (stars) & $8.75$ & $9.88$ & $4.30$ & $4.85$  \\
$\kappa=7/3$ (gas) & $8.03$ & $7.10$ & $4.34$ & $3.83$ \\
\hline
\end{tabular}


